$U$-statistics on bipartite exchangeable networks

Bipartite networks with exchangeable nodes can be represented by row-column exchangeable matrices. A quadruplet is a submatrix of size $2 \times 2$. A quadruplet $U$-statistic is the average of a function on a quadruplet over all the quadruplets of a matrix. We prove several asymptotic results for quadruplet $U$-statistics on row-column exchangeable matrices, including a weak convergence result in the general case and a central limit theorem when the matrix is also dissociated. These results are applied to statistical inference in network analysis. We suggest a method to perform parameter estimation, network comparison and motifs count for a particular family of row-column exchangeable network models: the bipartite expected degree distribution (BEDD) models. These applications are illustrated by simulations.

==> abstract.tex <==
$U$-statistics are used to estimate a population parameter by averaging a function on a subsample over all the subsamples of the population. In this paper, the population we are interested in is formed by the entries of a row-column exchangeable matrix. We consider $U$-statistics derived from functions of quadruplets, i.e. submatrices of size $2 \times 2$. We prove a weak convergence result for these $U$-statistics in the general case and we establish a Central Limit Theorem when the matrix is also dissociated. We shed further light on these results using the Aldous-Hoover representation theorem for row-column exchangeable random variables. Finally, to illustrate these results, we give examples of hypothesis testing for bipartite networks.

==> acknowledgements.tex <==
The author thanks Stéphane Robin (INRAE), Sophie Donnet (INRAE) and François Massol (CNRS) for many fruitful discussions and insights. This work was funded by a grant from Région Île-de-France and by the grant ANR-18-CE02-0010-01 of the French National Research Agency ANR (project EcoNet). 

==> applications.tex <==

In this section, we illustrate how to build statistical tests on RCE networks using our result. Indeed, $U$-statistics can be used to build unbiased estimators. The advantage of taking quadruplets is to define functions over several interactions of the same row or column. This allows us to extract information on the row and column distribution. Theorem~\ref{th:gaussian_theorem} then guarantees an asymptotic normality result, where the only unknown is $V$, which has to be estimated then plugged in with Slutsky's Theorem.

Now through different examples, we will show how one might use different kernels to estimate all the needed quantities to design tests on the Version 1 of the WBEDD (with constant density), to which Theorem~\ref{th:gaussian_theorem} applies.

\subsection{Heterogeneity in the row degrees of a network}

Remember that the function $f$ (resp. $g$) of the WBEDD model defines the expected weight distribution of the row (resp. column) nodes. For all $k > 0$, we denote $F_k = \int_0^1 f^k(u) du$ (resp. $G_k = \int_0^1 g^k(v) dv$). Consider that we are interested in the distribution of the row degrees only. We know that $F_1 = 1$, but we see that $F_2 = \int_0^1 f^2(u) du$ quantifies the heterogeneity in the row degrees. Indeed, if $f$ is constant, i.e. $f \equiv 1$ and $F_2 = 1$, then the row degrees are homogeneous. Besides, the higher $F_2$, the more unbalanced their distribution. More specifically, a large value of $F_2$ indicates a strong distinction between generalist (with high degree) and specialists (with low degree) nodes. Then in order to evaluate the homogeneity of the rows of a network, it makes sense to test the following hypotheses : $\mathcal{H}_0 : f \equiv 1$ vs. $\mathcal{H}_1 : f \not\equiv 1$ using an estimator of $F_2$.

$F_2$ can be estimated with the $U$-statistic based on the quadruplet kernel $h_1(Y_{[i_1,i_2;j_1,j_2]}) = \frac{1}{2}(Y_{i_1j_1}Y_{i_1j_2} + Y_{i_2j_1}Y_{i_2j_2})$. We see that $\mathbb{E}[U^{h_1}_N] = \mathbb{E}[h_1(Y_{\{i_1,i_2;j_1,j_2\}})] = \lambda^2 F_2$. So Theorem~\ref{th:gaussian_theorem} and the derivation of $V$ gives the following result :
\begin{equation*}
    \sqrt{\frac{N}{V}}(U^{h_1}_N - \lambda^2 F_2) \xrightarrow[N \rightarrow \infty]{\mathcal{D}} \mathcal{N}(0, 1),
\end{equation*}
where $V = \lambda^4 c^{-1} (F_4 - F_2^2) + 4 \lambda^4 (1-c)^{-1}  F_2^2 (G_2 - 1)$.

We use the kernel $h_2(Y_{\{i_1,i_2;j_1,j_2\}}) = \frac{1}{4}(Y_{i_1j_1} + Y_{i_1j_2} + Y_{i_2j_1} + Y_{i_2j_2})$ to construct $U^{h_2}_N$, a consistent estimator of $\lambda$. It follows from Slutsky's theorem that
\begin{equation}
    \sqrt{\frac{N}{V}} (U^{h_2}_N)^2 \bigg(\frac{U^{h_1}_N}{(U^{h_2}_N)^2} - F_2\bigg) \xrightarrow[N \rightarrow \infty]{\mathcal{D}} \mathcal{N}(0, 1).
    \label{eq:asymptotic_f2}
\end{equation}

Under $\mathcal{H}_0$, $F_2 = F_4 = 1$, so $V = 4 \lambda^4 (1-c)^{-1} (G_2 - 1)$. Then, to estimate $V$, we consider the $U$-statistic based on the kernel $h_3(Y_{[i_1,i_2;j_1,j_2]}) = \frac{1}{2}(Y_{i_1j_1}Y_{i_2j_1} + Y_{i_1j_2}Y_{i_2j_2})$, which is a consistent estimator for $\lambda^2 G_2$. Thus, $V$ can be consistently estimated by
\begin{equation*}
    \hat{V}_N = \frac{4}{1-c} (U^{h_2}_{N})^4 \left[ \frac{U^{h_3}_{N}}{(U^{h_2}_{N})^2} - 1\right].
\end{equation*}

Finally, a further application of Slutsky's theorem implies that under $\mathcal{H}_0$,
\begin{equation*}
    \sqrt{\frac{N}{\hat{V}_N}} (U^{h_2}_N)^2 \bigg(\frac{U^{h_1}_N}{(U^{h_2}_N)^2} - 1\bigg) \xrightarrow[N \rightarrow \infty]{\mathcal{D}} \mathcal{N}(0, 1).
\end{equation*}
This result allows us to define an asymptotic test for $\mathcal{H}_0 : F_2 = 1$.

\subsection{Network comparison}

The previous example shows how to build a test for a single network. In fact, it is easy to extend this framework to network comparison, provided the networks are independent. Indeed, say network $Y^A$ and $Y^B$ are independent. Then for any quadruplet kernel $h$, the $U$-statistics $U_N^h(Y^A)$ and $U_N^h(Y^B)$ computed on each network are also independent. Therefore, if we were to compare the row degree unbalance of two networks, we can opt for a test of the type $\mathcal{H}_0 : F^A_2 = F^B_2$ vs. $\mathcal{H}_1 : F^A_2 \neq F^B_2$. One can simply notice that $U_N^h(Y^A) - U_N^h(Y^B)$ is still asymptotically normal, with $\mathbb{E}[U_N^h(Y^A) - U_N^h(Y^B)] = F^A_2 - F^B_2$ and it is easy to find the asymptotic variance $V$ as $\mathbb{V}[U_N^h(Y^A) - U_N^h(Y^B)] = \mathbb{V}[U_N^h(Y^A)] + \mathbb{V}[U_N^h(Y^B)]$.

\subsection{Further remarks and leads}

We have showcased an example of application of our result to statistical test design. One interesting feature of the kernels used is that they are simple to compute. Indeed, if we denote $Y_N := (Y_{ij})_{1 \le i \le m_N, 1 \le j \le n_N}$, one can write the $U$-statistics used in the previous example as
\begin{equation*}
\begin{split}
    U^{h_1}_{N} &= \frac{1}{n_N m_N (m_N-1)} \left[ |Y_N^TY_N|_1 - \Trace(Y_N^TY_N)\right], \\
    U^{h_2}_{N} &= \frac{1}{n_N m_N} |Y_N|_1, \\
    U^{h_3}_{N} &= \frac{1}{n_N(n_N-1)m_N} \left[ |Y_NY_N^T|_1 - \Trace(Y_NY_N^T)\right],
\end{split}
\end{equation*}
where $\Trace$ is the trace operator. We see that these $U$-statistics can be computed using only simple operations on matrices, which are optimized in most computing software.

However, one can define more elaborate kernels to test further hypotheses on other models. The only conditions on the model are that it should be RCE and dissociated, i.e. it can be written as a bipartite W-graph model. For example, given the W-graph model $Y_{ij}~|~\xi_i, \eta_j \sim \mathcal{P}(\lambda w(\xi_i, \eta_j))$ with $\int \int w = 1$, one could have tested if it is of product form, i.e. if $f(u) = \int w(u,v) dv$ and $g(v) = \int w(u,v) du$, $w$ can be written as $w(u,v) = f(u) g(v)$ (as in the WBEDD model). An appropriated kernel for this test would be
\begin{equation*}
\begin{split}
    h(Y_{\{i_1, i_2; j_1, j_2\}}) =& \frac{1}{4}Y_{i_1j_1} Y_{i_2j_2}(Y_{i_1j_1} + Y_{i_2j_2} - Y_{i_1j_2} - Y_{i_1j_2} - 2) \\
    &+ \frac{1}{4}Y_{i_1j_2} Y_{i_1j_2} (Y_{i_1j_2} + Y_{i_1j_2} - Y_{i_1j_1} - Y_{i_2j_2} - 2)
\end{split}
\end{equation*}
as $\mathbb{E}[h(Y_{\{i_1, i_2; j_1, j_2\}})] = \int \int w(u,v)(w(u,v) - f(u)g(v)) du dv$ and should be equal to 0 if the hypothesis is true.

The counts of bipartite motifs of size $2 \times 2$ can be expressed as quadruplet $U$-statistics and can be integrated in our framework. If $Y$ is a binary matrix, then one can count the diagonal motifs using a kernel and obtain statistical guarantees. For example, motif 5 of Figure 7 in~\cite{ouadah2021motif} can be counted with the kernel
\begin{equation*}
\begin{split}
    h(Y_{\{i_1,i_2;j_1,j_2\}}) =& Y_{i_1j_1} Y_{i_1j_2} Y_{i_2j_1} (1 - Y_{i_2j_2}) + Y_{i_1j_1} Y_{i_1j_2} Y_{i_2j_2} (1 - Y_{i_2j_1}) \\
    &+ Y_{i_1j_1} Y_{i_2j_1} Y_{i_2j_2} (1 - Y_{i_1j_2}) + Y_{i_1j_2}Y_{i_2j_1} Y_{i_2j_2} (1 - Y_{i_1j_1}).
\end{split}
\end{equation*}

It is legitimate to wonder if one can extend our framework to $U$-statistics over submatrices of size different from $2 \times 2$, for example $Y_{\{i_1,...,i_{p};j_1,...,j_{q}\}}$ of size $p \times q$. If this can be done, then our framework can be used to count motifs of larger size. Also, one could have used formula~(\ref{eq:asymptotic_f2}) of the row heterogeneity example to derive an asymptotic confidence interval for $F_2$ (we do not necessarily have $F_2 = F_4 = 1$). Instead of using quadruplet kernels, we notice that one could have estimated the term $\lambda^4 F_4$ appearing in $V$ with a kernel over submatrices of size $1 \times 4$ such as $h(Y_{\{i_1; j_1, j_2,j_3,j_4\}}) = Y_{i_1j_1}Y_{i_1j_2}Y_{i_1j_3}Y_{i_1j_4}$ and $\mathbb{E}[h(Y_{\{i_1; j_1, j_2,j_3,j_4\}})] = \lambda^4 F_4$. The possibility for an extension is discussed in the next section.  



==> discussion.tex <==
We do not claim that the chosen kernels and the derived $U$-statistics necessarily lead to the most powerful tests. We have seen that one might combine several $U$-statistics to find a consistent estimator for $V$. Especially, this might make the convergence of $\hat{V}_N$ slow, especially when these $U$-statistics are correlated and there might exist more optimal kernels to build this test. In conclusion, these $U$-statistics based on quadruplets might not be theoretically the most efficient estimators, but more importantly, they are simple and easy to compute in practice.

It is possible to extend our theorem to $U$-statistics over submatrices of size different from $2 \times 2$, for example $Y_{\{i_1,...,i_{p};j_1,...,j_{q}\}}$ of size $p \times q$. In this case, for some kernel $h$ on these submatrices,
\begin{equation*}
  U^h_N = \left[\binom{m_N}{p}\binom{n_N}{q}\right]^{-1} \sum_{1\le i_1<...<i_{p}\le m_N} \sum_{1\le j_1<...<j_{q}\le n_N} h(Y_{\{i_1,...,i_{p};j_1,...,j_{q}\}}),
\end{equation*}
would also be asymptotically normal. All the steps of our proof can be adapted to $U$-statistics of larger subgraphs. These $U$-statistics are indeed backward martingales and the equivalent of Proposition~\ref{prop:asymptotic_variance} and Proposition~\ref{prop:lindeberg_condition} require more calculus. As a consequence, the asymptotic variance also has a different expression. On the one hand, such an extension would allow more flexibility in the choice of the kernel, hence the ability to build more complex estimators. On the other hand, in practice, the computation of such $U$-statistics may also be more complex and computationally demanding, whereas simple functions on quadruplets can easily be expressed with matrix operations. 

Further studies might be carried to investigate the rate of convergence of $\sqrt{N}(U^h_{N}-U^h_\infty)$ to its limiting distribution. A possible direction is the derivation of a Berry-Esseen-type bound. For specific applications, the computation of this rate through numerical simulation is also possible.

==> introduction.tex <==
$U$-statistics form a large class of statistics with powerful properties. They are built as the average of a given function on a subsample of a population, called kernel, applied to all the subsamples taken from this population. The population usually consists of i.i.d. individuals. In this case, \cite{hoeffding1948class} gives a Central Limit Theorem (CLT), which ensures their asymptotic normality. For non-i.i.d. cases, similar results~\citep{nandi1963properties} exist when the population is exchangeable, i.e. when the joint distribution of a subsample only depends on its size or equivalently for any finite permutation $\sigma$,
\begin{equation*}
    (Y_1, Y_2, ...) \overset{\mathcal{D}}{=} (Y_{\sigma(1)}, Y_{\sigma(2)}, ...).
\end{equation*}
In these cases, it is convenient to view the kernel $h$ taken on each subsample of size $k$ as a random variable indexed by $k$-tuple, e.g. $X_{\boldsymbol i} = X_{i_1 i_2 ... i_k} := h(Y_{i_1}, Y_{i_2}, ..., Y_{i_k})$ and the $U$-statistic is therefore a sum of random variables. If the population is exchangeable, then the array $X$ is not necessarily exchangeable, but it is jointly exchangeable, i.e. for any sequence of $k$-tuples $(\boldsymbol i, \boldsymbol j, ...)$ and for any finite permutation $\sigma$,
\begin{equation*}
    (X_{\boldsymbol i}, X_{\boldsymbol j}, ...) \overset{\mathcal{D}}{=} (X_{\sigma(i_1) \sigma(i_2) ... \sigma(i_k)}, X_{\sigma(j_1) \sigma(j_2) ... \sigma(j_k)}, ...).
\end{equation*}
A CLT exists for sums of jointly exchangeable variables, which has been proven by~\cite{eagleson1978limit}.

In our paper, the sample consists of the entries of a matrix $Y$ of size $m \times n$, the rows and columns of which are separately exchangeable (row-column exchangeable, RCE), i.e. denoting $\mathbb{S}_n$ the symmetric group of order $n$, for any $\Phi = (\sigma_1,\sigma_2) \in \mathbb{S}_m \times \mathbb{S}_n$, 
\begin{equation*}
    \Phi Y \overset{\mathcal{D}}{=} Y,
\end{equation*}
where $\Phi Y := (Y_{\sigma_1(i)\sigma_2(j)})_{1 \le i,j < \infty}$. We consider $U$-statistics based on submatrices of size $2 \times 2$, that we call quadruplets
\begin{equation*}
    Y_{\{i_1,i_2;j_1,j_2\}} := \left(
    \begin{matrix}
    Y_{i_1j_1} & Y_{i_1j_2} \\
    Y_{i_2j_1} & Y_{i_2j_2}
    \end{matrix}
    \right).
\end{equation*}
Their kernels are real functions $h$ such that for any matrix $Y$, $h(Y_{\{1,2;1,2\}}) = h(Y_{\{2,1;1,2\}}) = h(Y_{\{1,2;2,1\}})$. Applied to a matrix of size $m \times n$, a quadruplet $U$-statistic is then defined by 
\begin{equation*}
    U^h_{m,n} = \binom{m}{2}^{-1} \binom{n}{2}^{-1} \sum_{\substack{1 \le i_1 < i_2 \le m\\1 \le j_1 < j_2 \le n}} h(Y_{\{i_1,i_2;j_1,j_2\}}),
\end{equation*}
where $\binom{m}{2}$ is the number of $2$-combinations from $m$ elements. We can denote $X_{[i_1, i_2; j_1, j_2]} := h(Y_{\{i_1, i_2; j_1, j_2\}})$. However, contrarily to the case where $Y$ is fully exchangeable, $X$ is not jointly exchangeable in this case. Our aim is to establish a weak convergence theorem for these $U$-statistics using the martingale approach used by \cite{eagleson1978limit}.

We apply our results to network analysis. The matrix $Y$ can be seen as a weighted bipartite network, where the rows and the columns represent individuals of two different types, and the interactions can only happen between individuals of two different types. Each entry $Y_{ij}$ represents the intensity of the interaction between the individuals $i$ (of type 1) and $j$ (of type 2). As an example, we consider two versions of the Weighted Bipartite Expected Degree Distribution (WBEDD) model, which is a weighted, bipartite and exchangeable extension of the Expected Degree Sequence model~\citep{chung2002average, ouadah2021motif}. For binary graphs, the degree of a node is the number of edges that stem from it. For weighted graphs, the equivalent notion is the sum of the weights of these edges. It is sometimes called node strength~\citep{barrat2004architecture}, but we will simply refer to it as node weight. The WBEDD model draws the node weights from two distributions, characterised by real functions $f$ and $g$. The expected edge weights $Y_{ij}$ are then proportional to the expected weights of the involved nodes. The model can be written as
\begin{align*}
\begin{split}
    \xi_i, \eta_j &\overset{iid}{\sim} \mathcal{U}[0,1] \\ 
    Y_{ij}~|~\xi_i, \eta_j &\sim \mathcal{L}(\lambda f(\xi_i) g(\eta_j)).
\end{split}
\end{align*} 
where $\mathcal{L}$ is a family of probability distributions over positive real numbers such that the expectation of $\mathcal{L}(\mu)$ is $\mu$ and $f$ and $g$ are normalized by the condition $\int f = \int g = 1$. Consequently, $\lambda$ is the mean intensity of the network. The two versions of the WBEDD are: 
\begin{description}
    \item[Version 1] $\lambda$ is constant,
    \item[Version 2] $\lambda$ is a positive random variable.
\end{description}
We explain the implications of the two versions and how our results apply to both of them. Then we suggest a framework to design statistical tests on these models using our CLT and we discuss how one can extend it.

Our results are presented and proven in Section~\ref{sec:main}. In addition to the RCE case, we prove that if the matrix is also dissociated, i.e. if any of its submatrices with disjoint indexing sets are independent, then we obtain a CLT. Section~\ref{sec:app} gives examples of application of this CLT to hypothesis testing on networks. 

\iffalse
\subsection{Permutations and $U$-statistics}

Our results will apply in an asymptotic framework where the numbers of rows and columns of $Y$ grow at the same rate, i.e. ${m}/({m+n}) \rightarrow c$ and at each step, only one row or one column is added to the matrix $Y$. Now, we build a sequence of dimensions $(m_N, n_N)_{N \ge 1}$ that satisfies these conditions.

\begin{definition}[Sequences of dimensions] \label{def:mn}
    Let $c$ be an irrational number such that $0<c<1$. For all $N \in \mathbb{N}$, we define $m_N = 2 + \lfloor c(N+1) \rfloor$ and $n_N = 2 + \lfloor (1-c)(N+1) \rfloor$, where $\lfloor \cdot \rfloor$ is the floor function.
\end{definition}

\begin{proposition}
    $m_N$ and $n_N$ satisfy: 
    \begin{enumerate}
        \item $\frac{m_N}{m_N + n_N} \underset{N \rightarrow \infty}{\longrightarrow} c$,
        \item $m_N + n_N = 4 + N$, for all $N \in \mathbb{N}$.
    \end{enumerate}
    \label{prop:sequences}
\end{proposition}

\begin{corollary}
    At each iteration $N \in \mathbb{N}^*$, one and only one of these two propositions is true:
    \begin{enumerate}
        \item $m_N = m_{N-1} + 1$ and $n_N = n_{N-1}$,
        \item $n_N = n_{N-1} + 1$ and $m_N = m_{N-1}$.
    \end{enumerate}
    \label{cor:partition}
\end{corollary}

Such sequences $m_N$ and $n_N$ satisfy the desired growth conditions (proof given in Appendix~\ref{app:mn}). We define the sequence of $U$-statistics as $U^h_{N} := U^h_{m_N, n_N}$.

\subsection{RCE matrices}

Our result stems from the fact that we will be considering row-column exchangeable matrices. These random matrices have distributions that are invariant under row-column permutations that we define as follows.

\begin{notation*}[Groups of permutations] 
    We denote $\mathbb{S}_n$ the symmetric group of order $n$, i.e. the group of permutations over $\mathbb{N}^*$ that only act on the first $n$ integers.
\end{notation*}

\begin{notation*}[Row-column permutation on a matrix]
    Let $\Phi = (\sigma_1,\sigma_2) \in \mathbb{S}_m \times \mathbb{S}_n$. For a matrix $Y$ of size $m \times n$, we denote
    \begin{equation*}
        \Phi Y := (Y_{\sigma_1(i)\sigma_2(j)})_{1 \le i,j < \infty}
    \end{equation*}
\end{notation*}

\begin{definition}[RCE matrix]
   Let  $Y$ be a random matrix of size $m \times n$. $Y$ is said to be a row-column exchangeable (RCE) matrix  if and only if for all $\Phi \in \mathbb{S}_m \times \mathbb{S}_n$,
    \begin{equation*}
        \Phi Y \overset{\mathcal{D}}{=} Y.
    \end{equation*}
\end{definition}

For ease of interpretation, it is convenient to imagine the rectangular matrix as a weighted bipartite network, where the rows and the columns represent individuals of two different types, and the interactions can only happen between individuals of two different types. Each value $Y_{ij}$ represents the intensity of the interaction between the individuals $i$ (of type 1) and $j$ (of type 2). 

To illustrate our paper, we will consider two versions of the Weighted Bipartite Expected Degree Distribution (WBEDD) model, which are weighted, bipartite and exchangeable variations of the expected degree distribution model~\shortcite{chung2002average, picard2008assessing}. For binary graphs, the degree of a node is the number of edges that stem from it. For weighted graphs, the equivalent notion is the sum of the weights of the edges. It is sometimes called node strength~\shortcite{barrat2004architecture}, but we will simply refer to it as node weight. The WBEDD model draws the node weights from two distributions, characterised by real functions $f$ and $g$. The expected edge weights $Y_{ij}$ are then proportional to the expected weights of the involved nodes. The model can be written as
\begin{align}
\begin{split}
    \xi_i, \eta_j &\overset{iid}{\sim} \mathcal{U}[0,1] \\ 
    Y_{ij}~|~\xi_i, \eta_j &\sim \mathcal{L}(\lambda f(\xi_i) g(\eta_j)).
\end{split}
\end{align} 
where $\mathcal{L}$ is a family of positive probability distributions such that the expectation of $\mathcal{L}(\mu)$ is $\mu$ and $f$ and $g$ are normalized by the condition $\int f = \int g = 1$. Consequently, $\lambda$ is the mean intensity of the network.

Now we consider the following two versions of the WBEDD : 
\begin{itemize}
    \item \textbf{Version 1} $\lambda$ is constant,
    \item \textbf{Version 2} $\lambda$ is a random variable following a positive probability distribution.
\end{itemize}
We will see the implications of the two versions and how our results apply to both of them.
\fi

==> main-result.tex <==
\subsection{Asymptotic framework}

Our results apply in an asymptotic framework where the numbers of rows and columns of $Y$ grow at the same rate, i.e. ${m}/({m+n}) \rightarrow c$ and at each step, only one row or one column is added to the matrix $Y$. Now, we build a sequence of dimensions $(m_N, n_N)_{N \ge 1}$ that satisfies these conditions.

\begin{definition}[Sequences of dimensions] \label{def:mn}
    Let $c$ be an irrational number such that $0<c<1$. For all $N \in \mathbb{N}$, we define $m_N = 2 + \lfloor c(N+1) \rfloor$ and $n_N = 2 + \lfloor (1-c)(N+1) \rfloor$, where $\lfloor \cdot \rfloor$ is the floor function.
\end{definition}

\begin{proposition}
    $m_N$ and $n_N$ satisfy: 
    \begin{enumerate}
        \item $\frac{m_N}{m_N + n_N} \xrightarrow[N \rightarrow \infty]{} c$,
        \item $m_N + n_N = 4 + N$, for all $N \in \mathbb{N}$.
    \end{enumerate}
    \label{prop:sequences}
\end{proposition}

\begin{corollary}
    At each iteration $N \in \mathbb{N}^*$, one and only one of these two propositions is true:
    \begin{enumerate}
        \item $m_N = m_{N-1} + 1$ and $n_N = n_{N-1}$,
        \item $n_N = n_{N-1} + 1$ and $m_N = m_{N-1}$.
    \end{enumerate}
    \label{cor:partition}
\end{corollary}

Such sequences $m_N$ and $n_N$ satisfy the desired growth conditions (proof given in Appendix~\ref{app:mn}). We define the sequence of $U$-statistics as $U^h_{N} := U^h_{m_N, n_N}$.

\subsection{Theorems}

We establish the following results on the asymptotic behaviour of $U$-statistics over RCE matrices.

\begin{theorem}[Main theorem]
    Let $Y$ be a RCE matrix. Let $h$ be a quadruplet kernel such that $\mathbb{E}[h(Y_{\{1,2;1,2\}})^2] < \infty$. Let $\mathcal{F}_N = \sigma\big((U^h_{kl}, k \ge m_N, l \ge n_N)\big)$ and $\mathcal{F}_\infty := \bigcap_{N = 1}^{\infty} \mathcal{F}_N$. Set $U^h_\infty = \mathbb{E}[h(Y_{\{1,2;1,2\}})|\mathcal{F}_\infty]$. Then
    \begin{equation*}
        \sqrt{N}(U^h_{N}-U^h_\infty) \xrightarrow[N \rightarrow \infty]{\mathcal{D}} W,
    \end{equation*}
    where $W$ is a random variable with characteristic function $\phi(t) = \mathbb{E}[\exp(-\frac{1}{2} t^2 V)]$, where
    \begin{equation*}
        V = \frac{4}{c}\Cov\big(h(Y_{\{1,2;1,2\}}),h(Y_{\{1,3;3,4\}}) \big|\mathcal{F}_\infty \big) + \frac{4}{1-c}\Cov\big(h(Y_{\{1,2;1,2\}}),h(Y_{\{3,4;1,3\}})\big|\mathcal{F}_\infty \big).
    \end{equation*}
    \label{th:mixture_theorem}
\end{theorem}

Theorem~\ref{th:mixture_theorem} states that the limit distribution of $\sqrt{N}(U^h_N - U^h_\infty)$ is a mixture of Gaussians, but we see that if $V$ is constant, then it is a simple Gaussian. Next we identify a class of models where the limiting distribution of $\sqrt{N}(U^h_N - U^h_\infty)$ is a simple Gaussian. 

\begin{definition}
  $Y$ is a dissociated matrix if and only if $(Y_{ij})_{1 \le i \le m, 1 \le j \le n}$ is independent of $(Y_{ij})_{i > m, j > n}$, for all $m$ and $n$.
\end{definition}

In other words, $Y$ is dissociated if submatrices that are not sharing any row or column are independent. Now we claim the following extension to Theorem~\ref{th:mixture_theorem} for dissociated RCE matrices.

\begin{theorem}
    In addition to the hypotheses of Theorem~\ref{th:mixture_theorem}, if $Y$ is dissociated, then $U^h_\infty$ and $V$ are constant and \begin{equation*}
        \sqrt{N}(U^h_{N}-U^h_\infty) \xrightarrow[N \rightarrow \infty]{\mathcal{D}} \mathcal{N}(0, V),
    \end{equation*}
    More precisely,
    \begin{enumerate}
        \item $U^h_\infty = \mathbb{E}[h(Y_{\{1,2;1,2\}})]$,
        \item $V = \frac{4}{c}\Cov\big(h(Y_{\{1,2;1,2\}}),h(Y_{\{1,3;3,4\}})\big) + \frac{4}{1-c}\Cov\big(h(Y_{\{1,2;1,2\}}),h(Y_{\{3,4;1,3\}})\big)$.
    \end{enumerate}
    \label{th:gaussian_theorem}
\end{theorem}

Now we shall explain this result in the light of the Aldous-Hoover representation theorem. Theorem 1.4 of~\cite{aldous1981representations} states that for any RCE matrix $Y$, there exists a real function $f$ such that if we denote $Y^*_{ij} = f(\alpha, \xi_i, \eta_j, \zeta_{ij})$, for $1 \le i,j < \infty$, where the $\alpha$, $\xi_i$, $\eta_j$ and $\zeta_{ij}$ are i.i.d. random variables with uniform distribution over $[0,1]$, then
\begin{equation*}
    Y \overset{\mathcal{D}}{=} Y^*.
\end{equation*}

It is possible to identify the role of each of the random variables involved in the representation theorem. We notice that each $Y_{ij}$ is determined by $\alpha, \xi_i, \eta_j$ and $\zeta_{ij}$. $\zeta_{ij}$ is entry-specific while $\xi_i$ is shared by all the entries involving the row $i$ and $\eta_j$ by the ones involving the column $j$. Therefore, the $\xi_i$ and $\eta_j$ represent the contribution of each individual of type 1 and type 2 of the network, i.e. each row and column of the matrix. These contributions are i.i.d., which makes the network exchangeable. Finally, $\alpha$ is global to the whole network and shared by all entries.

Proposition 3.3 of~\cite{aldous1981representations} states that if $Y$ is dissociated, then $Y^*$ can be written without $\alpha$, i.e. it is of the form $Y^*_{ij} = f(\xi_i, \eta_j, \zeta_{ij})$, for $1 \le i,j < \infty$. In this case, because the $\xi_i$, $\eta_j$ and $\zeta_{ij}$ are i.i.d., averaging with the $U$-statistic over an increasing number of nodes nullifies the contribution of each individual interaction ($\zeta_{ij}$) and node ($\xi_i$ and $\eta_j$). In the general case, i.e. when $Y$ is not dissociated, then conditionally on $\alpha$, $Y$ is dissociated. It is easy to see that the mixture of Gaussians from Theorem~\ref{th:mixture_theorem} results from this conditioning.

We can also state with ease that Theorem~\ref{th:mixture_theorem} can be applied to matrices $Y$ generated by the two versions of the WBEDD model. Theorem~\ref{th:gaussian_theorem} only applies to Version 1, where the matrix is dissociated. Indeed, we see that in both models conditionally on $\lambda$, the expected mean of the interactions of any submatrix is $\lambda$. Therefore any 2 submatrices are independent if $\lambda$ is constant. We could also have noticed that $\lambda$ is determined by the $\alpha$ from the representation theorem of Aldous-Hoover.

In practice, dissociated exchangeable random graph models are widely spread. Notably, a RCE model is dissociated if and only if it can be written as a $W$-graph (or graphon), i.e. it is defined by a distribution $\mathcal{W}$ depending on two parameters in $[0,1]$ such that for $1 \le i,j < \infty$ :
\begin{equation*}
  \begin{split}
    \xi_i, \eta_j &\overset{i.i.d.}{\sim} \mathcal{U}[0,1] \\
    Y_{ij}~|~\xi_i, \eta_j &\sim \mathcal{W}(\xi_i, \eta_j)
  \end{split}
\end{equation*}
In this definition, it is easy to recognize the variables from the representation theorem of Aldous-Hoover. We simply identify the $\xi_i$ and $\eta_j$, then it suffices to take $\phi^{-1}_{\xi_i, \eta_j}$ the inverse distribution function of $\mathcal{W}(\xi_i, \eta_j)$ to see that defining the dissociated RCE matrix $Y^*$ such that $Y^*_{ij} = f(\xi_i, \eta_j, \zeta_{ij}) := \phi^{-1}_{\xi_i, \eta_j}(\zeta_{ij})$ fulfills $Y^* \overset{\mathcal{D}}{=} Y$. It is also straightforward to remark that unlike Version 2, Version 1 of the WBEDD model can be written as a $W$-graph model, setting $\mathcal{W}(\xi_i, \eta_j) := \mathcal{L}(\lambda f(\xi_i) g(\eta_j))$. 


\subsection{Proof of Theorem~\ref{th:mixture_theorem}}

To prove Theorem~\ref{th:mixture_theorem}, we adapt the proof of \cite{eagleson1978limit} establishing the asymptotic normality of sums of backward martingale differences. The definition of a backward martingale is reminded in Appendix~\ref{app:backward}.

\begin{theorem}[\citealp{eagleson1978limit}]
    Let $(M_n, \mathcal{F}_n)_{n \ge 1}$ be a square-integrable reverse martingale, $V$ a $\mathcal{F}$-measurable, a.s. finite, positive random variable. Denote $M_\infty := \mathbb{E}[M_1 | \mathcal{F}_\infty]$ where $\mathcal{F}_\infty := \bigcap_{n = 1}^{\infty} \mathcal{F}_n$. Set $Z_{nk} := \sqrt{n}(M_k - M_{k+1})$. If:
    \begin{enumerate}
        \item $\sum_{k=n}^\infty \mathbb{E}[Z_{nk}^2 | \mathcal{F}_{k+1}] \xrightarrow[n \rightarrow \infty]{\mathbb{P}} V$ \text{(asymptotic variances)},
        \item for all $\epsilon > 0$, $\sum_{k=n}^\infty \mathbb{E}[Z_{nk}^2 \mathds{1}_{\{ |Z_{nk}| > \epsilon\}} | \mathcal{F}_{k+1}] \xrightarrow[n \rightarrow \infty]{\mathbb{P}} 0$ \text{(conditional Lindeberg condition)},
    \end{enumerate}
    then $\sum_{k=n}^\infty Z_{nk} = \sqrt{n}(M_n - M_\infty) \xrightarrow[n \rightarrow \infty]{\mathcal{D}} W$, where $W$ is a random variable with characteristic function $\phi(t) = \mathbb{E}[\exp(-\frac{1}{2} t^2 V)]$.
    \label{th:eagleson}
\end{theorem}

\begin{proof}[Proof of Theorem~\ref{th:mixture_theorem}]
    The three steps to apply Theorem~\ref{th:eagleson} to $(M_N)_{N \geq 1} = (U^h_N)_{N \geq 1}$ are to show that it is a backward martingale for a well chosen filtration and that it fulfills conditions $1$ and $2$. The expression of $V$ is made explicit along the way. More precisely, 
    \begin{enumerate}
        \item first, defining $\mathcal{F}_N = \sigma\big((U^h_{kl}, k \ge m_N, l \ge n_N)\big)$, Proposition~\ref{prop:martingale} states that $(U^h_N, \mathcal{F}_N)_{N \ge 1}$ is indeed a square-integrable reverse martingale ;
        \item then, Proposition~\ref{prop:asymptotic_variance} implies that $\sum_{k=n}^\infty \mathbb{E}[Z_{NK}^2 | \mathcal{F}_{K+1}]$ does converge to a random variable $V$ with the desired expression ;
        \item finally, the conditional Lindeberg condition is ensured by Proposition~\ref{prop:lindeberg_condition}, since  from it, we deduce that for all $\epsilon > 0$, $\sum_{K=N}^\infty \mathbb{E}[Z_{NK}^2 \mathds{1}_{\{ |Z_{NK}| > \epsilon\}} | \mathcal{F}_{K+1}] \xrightarrow[N \rightarrow \infty]{\mathbb{P}} 0$.
    \end{enumerate}
    Hence Theorem~\ref{th:eagleson} can be applied to $U^h_N$ and we obtain that $\sqrt{N}(U^h_N - U^h_\infty) \xrightarrow[N \rightarrow \infty]{\mathcal{D}} W$, where $W$ is a random variable with characteristic function $\phi(t) = \mathbb{E}[\exp(-\frac{1}{2} t^2 V)]$ with $V$ specified by Proposition~\ref{prop:asymptotic_variance}. The proofs of Propositions~\ref{prop:martingale}, ~\ref{prop:asymptotic_variance} and ~\ref{prop:lindeberg_condition}  are provided in Appendices~\ref{app:square},~\ref{app:variance}. and~\ref{app:lindeberg} respectively.
\end{proof}

\subsection{Proof of Theorem~\ref{th:gaussian_theorem}}

The proof of Theorem~\ref{th:gaussian_theorem} relies on a Hewitt-Savage type zero-one law for events that are permutable in our row-column setup. Therefore, it is useful to define first what a row-column permutable event is. We remind the Aldous-Hoover representation theorem for dissociated RCE matrices as stated earlier: if $Y$ is a dissociated RCE matrix, then its distribution can be written with $(\xi_i)_{1 \le i < m_N}$, $(\eta_j)_{1 \le j < n_N}$ and $(\zeta_{ij})_{1 \le i \le m_N, 1 \le j \le n_N}$ arrays of i.i.d. random variables.

Then let us consider such arrays of i.i.d. random variables $(\xi_i)_{1 \le i < m_N}$, $(\eta_j)_{1 \le j < n_N}$ and $(\zeta_{ij})_{1 \le i \le m_N, 1 \le j \le n_N}$. If we were to consider events depending only on them, there is no loss of generality in using the product probability space $(\Omega_N, \mathcal{A}_N, \mathbb{P}_N)$, where
\begin{equation*}
    \begin{split}
        \Omega_N &= \left\{ (\omega^\xi, \omega^\eta, \omega^\zeta) : \omega^\xi \in \mathbb{R}^{m_N}, \omega^\eta \in \mathbb{R}^{n_N}, \omega^\zeta \in \mathbb{R}^{m_N n_N} \right\} = \mathbb{R}^{m_N + n_N + m_N n_N}, \\
        \mathcal{A}_N &= \mathcal{B}(\mathbb{R})^{m_N + n_N + m_N n_N}, \\
        \mathbb{P}_N &= \mu^{m_N + n_N + m_N n_N}.
    \end{split}
\end{equation*}
We then define the action of a row-column permutation on an element of $\Omega_N$.
\begin{definition}
  Let $\Phi = (\sigma_1, \sigma_2) \in \mathbb{S}_{m_N} \times \mathbb{S}_{n_N}$. The action of $\Phi$ on $\omega \in \Omega_N$ is defined by
  \begin{equation*}
      \Phi \omega = \big(\sigma_1 \omega^\xi, \sigma_2 \omega^\eta, (\sigma_1,\sigma_2) \omega^\zeta\big)
  \end{equation*}
  where $\sigma_1 \omega^\xi = (\omega^\xi_{\sigma_1(i)})_{1 \le i < m_N}$, $\sigma_2 \omega^\eta = (\omega^\eta_{\sigma_2(j)})_{1 \le j < n_N}$ and $(\sigma_1,\sigma_2) \omega^\zeta = (\omega^\zeta_{\sigma_1(i) \sigma_2(j)})_{1 \le i < m_N, 1 \le j < n_N}$
\end{definition}

\begin{definition}
  Let $A \in \mathcal{A}_N$. $A$ is invariant by the action of $\mathbb{S}_{m_N} \times \mathbb{S}_{n_N}$ if and only if for all $\Phi \in \mathbb{S}_{m_N} \times \mathbb{S}_{n_N}$, $\Phi^{-1} A = A$, i.e.
  \begin{equation*}
      \left\{ \omega : \Phi \omega \in A \right\} = \left\{ \omega : \omega \in A \right\}.
  \end{equation*}
\end{definition}

\begin{notation*}
  In this section, we denote by $\mathcal{E}_N$ the collection of events of $\mathcal{A}_N$ that are invariant by row-column permutations of size $m_N \times n_N$, i.e. $\Phi \in \mathbb{S}_{m_N} \times \mathbb{S}_{n_N}$. We denote $\mathcal{E}_\infty := \bigcap_{n = 1}^{\infty} \mathcal{E}_N$, which is the collection of events that are invariant by permutations of size $m_N \times n_N$, for all $N$.
\end{notation*}

The following theorem is an extension of the Hewitt-Savage zero-one law to the row-column setup. 
\begin{theorem}
  For all $A \in \mathcal{E}_\infty$, $\mathbb{P}(A) = 0$ or $\mathbb{P}(A) = 1$.
  \label{th:hewitt_savage}
\end{theorem}

The proof of Theorem~\ref{th:hewitt_savage} is given in Appendix~\ref{app:normality}. Now we use this result to derive Theorem~\ref{th:gaussian_theorem} from Theorem~\ref{th:mixture_theorem}.

\begin{proof}[Proof of Theorem~\ref{th:gaussian_theorem}]
  In this proof, we specify the matrices over which the $U$-statistics are taken, i.e. we denote $U^h_{k,l}(Y)$ instead of $U^h_{k,l}$ the $U$-statistic of size $k \times l$ with kernel $h$ taken on $Y$. We denote also $\mathcal{F}_N(Y) = \sigma\big((U^h_{kl}(Y), k \ge m_N, l \ge n_N)\big)$ which are sets of events depending on $Y$.

  Since $Y$ is RCE and dissociated, Proposition 3.3 of~\cite{aldous1981representations} allows us to consider a real function $f$ such that for $1 \le i,j < \infty$, $Y^*_{ij} = f(\xi_i, \eta_j, \zeta_{ij})$ and $Y^* \overset{\mathcal{D}}{=} Y$, where  $\xi_i$, $\eta_j$ and $\zeta_{ij}$, for $1 \le i,j < \infty$ are i.i.d. random variables with uniform distribution on $[0,1]$. Therefore we can consider these random variables, the product spaces $(\Omega_N, \mathcal{A}_N, \mathbb{P}_N)$ and the sets $\mathcal{E}_N$ of invariant events defined earlier.
  
  But $\mathcal{F}_N(Y^*) = \sigma\big((U^h_{kl}(Y^*), k \ge m_N, l \ge n_N)\big) \subset \sigma(U_N(Y^*), \xi_i, \eta_j, \zeta_{ij}, i > m_N, j > n_N)$, so for all $N$, $\mathcal{F}_N(Y^*) \subset \mathcal{E}_N$. It follows that $\mathcal{F}_\infty(Y^*) \subset \mathcal{E}_\infty$, so $U_\infty(Y^*)$ is $\mathcal{F}_\infty(Y^*)$-measurable. Theorem~\ref{th:hewitt_savage} states that all the events in $\mathcal{E}_\infty$ happen with probability 0 or 1, so it ensures that $U_\infty(Y^*) = \mathbb{E}[h(Y^*_{\{1,2;1,2\}})|\mathcal{F}_\infty(Y^*)] = \mathbb{E}[h(Y^*_{\{1,2;1,2\}})]$ is constant. Moreover, since the distribution of $U^h_{N}(Y)$ is the same as this of $U^h_{N}(Y^*)$, we can conclude that $U_\infty(Y) = \mathbb{E}[h(Y_{\{1,2;1,2\}})|\mathcal{F}_\infty(Y)] = \mathbb{E}[h(Y_{\{1,2;1,2\}})]$. 
  
  Likewise, we deduce that $\mathbb{E}[h(Y_{\{1,2;1,2\}})h(Y_{\{1,3;3,4\}})|\mathcal{F}_\infty(Y)] = \mathbb{E}[h(Y_{\{1,2;1,2\}})h(Y_{\{1,3;3,4\}})]$ and $\mathbb{E}[h(Y_{\{1,2;1,2\}})h(Y_{\{3,4;1,3\}})|\mathcal{F}_\infty(Y)] = \mathbb{E}[h(Y_{\{1,2;1,2\}})h(Y_{\{3,4;1,3\}})]$ which gives the desired result for $V$. Thus we conclude that $W$ of Theorem~\ref{th:mixture_theorem} follows a Gaussian distribution of variance $V$.
  
\end{proof}


